Optimized Couplings for Watermarking Large Language Models

Large-language models (LLMs) are now able to produce text that is, in many cases, seemingly indistinguishable from human-generated content. This has fueled the development of watermarks that imprint a ``signal'' in LLM-generated text with minimal perturbation of an LLM's output. This paper provides an analysis of text watermarking in a one-shot setting. Through the lens of hypothesis testing with side information, we formulate and analyze the fundamental trade-off between watermark detection power and distortion in generated textual quality. We argue that a key component in watermark design is generating a coupling between the side information shared with the watermark detector and a random partition of the LLM vocabulary. Our analysis identifies the optimal coupling and randomization strategy under the worst-case LLM next-token distribution that satisfies a min-entropy constraint. We provide a closed-form expression of the resulting detection rate under the proposed scheme and quantify the cost in a max-min sense. Finally, we provide an array of numerical results, comparing the proposed scheme with the theoretical optimum and existing schemes, in both synthetic data and LLM watermarking. Our code is available at https://github.com/Carol-Long/CC_Watermark

==> isit_preamble.tex <==
%!TEX root = main.tex

\usepackage[usenames,dvipsnames]{xcolor}
%\usepackage{mdframed}
%\usepackage{bm}
%\usepackage{bbm}
\usepackage{dsfont}
\usepackage{amsbsy}
\usepackage{amssymb}
\usepackage{amsmath}%
\usepackage{amsfonts}%
\usepackage{amsthm}
\usepackage{breqn}
\usepackage{graphicx}
\usepackage{colonequals}
\usepackage{psfrag}
\usepackage{mathrsfs}
\usepackage[noadjust]{cite}
\usepackage{hyperref}
\usepackage{mdframed}
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{braket}
\usepackage{mathtools}

\usepackage[backgroundcolor=blue!15]{todonotes}


%Enumitem setting
\newcommand\litem[1]{\item{\bfseries #1:}}


\allowdisplaybreaks

\newtheorem{thm}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{prop}{Proposition}
\newtheorem{conj}{Conjecture}
\newtheorem{cor}{Corollary}
\newtheorem{assumptions}{Assumption}
\newtheorem{question}{Question}

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother
\newreptheorem{conj}{Conjecture}

%% For watermarking
\newcommand{\rd}{R_d}
\newcommand{\rp}{R_p}
\newcommand{\Qx}{Q_X} % LLM distribution
\newcommand{\tilqs}{\tilde{Q}_{X|S}} % watermark distribution
\newcommand{\tilqBm}{\tilde{Q}_{X|B^m}} % watermark distribution
\newcommand{\tilq}{\tilde{Q}_{X}} % marginalized watermarked distribution

\newcommand{\pbm}{p(b^m)} %no rnadomness
\newcommand{\pBm}{p(B^m)} %random variable
\newcommand{\tpbm}{\tilde{p}(b^m)} %no rnadomness
\newcommand{\tpBm}{\tilde{p}(B^m)} %random variable

%% Definition Styles
\theoremstyle{definition}
\newtheorem{quest}{Question}
\newtheorem{defn}{Definition}
\newtheorem{scheme}{Scheme}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
%%
\newcommand{\SNR}{\mbox{SNR}}
\newcommand{\dB}{\mbox{dB}}
\newcommand{\emu}{\colonsim}
\newcommand{\etal}{\textit{et al.}~}
\newcommand{\Fq}{\mathbb{F}_{q}}
%\newcommand{\PR}[1]{\mbox{Pr}\left\{ #1 \right\}}
\newcommand{\PR}{\mbox{Pr}}
\newcommand{\Lh}{\hat{l}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\Xk}{\mathcal{X}^k}
\newcommand{\Xn}{\mathcal{X}^n}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\mean}{\mathbb{E}}
\newcommand{\bc}{\mathbf{c}}

\newcommand{\fib}{f_{\mathsf{IB}}}
\newcommand{\fpf}{f_{\mathsf{PF}}}
\newcommand{\conv}{\mathsf{conv}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\rank}{\mbox{rank}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bbz}{\mathbf{z}}
\newcommand{\binstr}{\{0,1\}} 
\newcommand{\supp}{\mbox{supp}}
\renewcommand{\tilde}{\widetilde}
\newcommand{\Enc}{\mathsf{Enc}}
\newcommand{\Dec}{\mathsf{Dec}}
\newcommand{\Adv}{\mathsf{Adv}}
\newcommand{\chis}{\chi^2}
\newcommand{\Xh}{\hat{X}}
\newcommand{\Zh}{\hat{Z}}
\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\newcommand{\brk}[1]{\langle #1 \rangle}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\normQ}[1]{\| #1 \|_Q}
\newcommand{\normF}[1]{\| #1 \|_F}
\newcommand{\normX}[2]{\| #1 \|_{#2}}
\newcommand{\normEuc}[1]{\| #1 \|_2}
\newcommand{\ox}{\bar{x}}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\inertia}{\mathcal{I}}
\newcommand{\defined}{\triangleq}
\newcommand{\Tr}[1]{\mathrm{ tr}\left(#1 \right)}
\newcommand{\diag}[1]{\mathrm{diag}\left( #1 \right)}
\newcommand{\pxy}{P_{X,Y}}
\newcommand{\px}{P_X}
\newcommand{\py}{P_Y}
\newcommand{\pxp}{p_{X'}}
\newcommand{\pxgy}{P_{X|Y}}
\newcommand{\pygx}{P_{Y|X}}
\newcommand{\pbgx}{p_{B|X}}
\newcommand{\Ppygx}[1]{\mathbf{p}_{Y|X={#1}}}
\newcommand{\pxhgx}{p_{\Xh|X}}
\newcommand{\qx}{q_X}


\newcommand{\rx}{r_X}
\newcommand{\ExpVal}[2]{\mathbb{E}_{#1}\left[ #2 \right]}
\newcommand{\Mopt}{M_{\mathrm{ML}}}
\newcommand{\tZ}{\tilde{Z}}
\newcommand{\tU}{\tilde{U}}
\newcommand{\tV}{\tilde{V}}
\newcommand{\tsigma}{\tilde{\sigma}}
\newcommand{\Pxy}{\mathbf{P}_{X,Y}}
\newcommand{\Pxnyn}{P_{X^n,Y^n}}
\newcommand{\Pxyp}{P_{X',Y'}}
\newcommand{\Pygx}{\mathbf{P}_{Y|X}}
\newcommand{\Pxxp}{\bP_{X,\Xh}}
\newcommand{\Pxhgx}{P_{\hat{X}|X}}
\newcommand{\Px}{\mathbf{p}_X}
\newcommand{\Rx}{\mathbf{r}_X}
\newcommand{\Pxp}{\mathbf{p}_{\Xh}}
\newcommand{\Py}{\mathbf{p}_Y}
\newcommand{\At}{\tilde{\mathbf{A}}}
\newcommand{\Bt}{\tilde{\mathbf{B}}}
\newcommand{\Ut}{\tilde{\mathbf{U}}}
\newcommand{\Vt}{\mathbf{\tilde{V}}}
\newcommand{\Yt}{\tilde{Y}}
\newcommand{\Zt}{\tilde{Z}}
\newcommand{\lambdat}{\tilde{\lambda}}
\newcommand{\Sigmat}{\tilde{\mathbf{\Sigma}}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\Lb}{L}
\newcommand{\blambda}{\pmb{\lambda}}
\newcommand{\blambdat}{\tilde{\pmb{\lambda}}}
\newcommand{\bLambda}{\pmb{\Lambda}}
\newcommand{\Emat}{\mathbf{F}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\btu}{\tilde{\mathbf{u}}}
\newcommand{\btv}{\tilde{\mathbf{v}}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\tv}{\tilde{v}}
\newcommand{\olU}{\overline{\mathbf{U}}}
\newcommand{\deriv}[2]{\frac{\delta #1}{\delta #2}}
\newcommand{\sto}{\mbox{\normalfont s.t.}}
\newcommand{\KFnorm}[2]{\| #1 \|_{#2}}
\newcommand{\Imeas}{J}
\newcommand{\bigO}{O}
\newcommand{\ttheta}{\tilde{\theta}}
\newcommand{\Var}[2]{\mathrm{Var}_{#1}#2 }
\newcommand{\whf}{\widehat{f}}
\newcommand{\whg}{\widehat{g}}
\newcommand{\ft}{\tilde{f}}
\newcommand{\Yh}{\widehat{Y}}
%\newcommand{\pbgx}{p_{B|X^n}}
\newcommand{\pbgy}{p_{B|Y^n}}
\newcommand{\whh}{\widehat{h}}
% \newcommand{\EE}[1]{\ExpVal{}{#1}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\EM}[2]{\ExpVal{#1}{#2}}
\newcommand{\whB}{\widehat{B}}
\newcommand{\wbeta}{\widehat{\beta}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\eye}{\mathbf{I}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bSigma}{\mathbf{\Sigma}}
\newcommand{\bsigma}{\boldsymbol\sigma}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bbH}{\mathbf{H}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\suchthat}{\,\mid\,}
\newcommand{\indicator}{\mathds{1}}
\newcommand{\mmse}{\mathsf{mmse}}
\newcommand{\error}{\mathsf{e}}
%%
\newcommand{\calN}{\mathcal{N}}
\newcommand{\cwd}{\{1,\dots,2^{nR} \}}
\newcommand{\Ps}{\mathbf{p}_S}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\TV}{\mathsf{TV}}
\newcommand{\lse}{\mathsf{lmmse}}
\newcommand{\dks}{d_{\mathrm{KS}}}
\newcommand{\Xt}{\widetilde{X}}
\newcommand{\xh}{\hat{x}}
\newcommand{\vs}{v^*(p_{S,X})}
\newcommand{\dps}{\delta(p_{S,X})}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\simplex}{\Delta}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\KC}{\calJ}
\newcommand{\Fsym}{\calF_{\mathrm{sym}}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\Dx}{\mathbf{D}_X}
\newcommand{\Dy}{\mathbf{D}_Y}
\newcommand{\Dkl}{\mathsf{D}_{\mathsf{KL}}}
\newcommand{\pdset}{\calP^m_{++}}
\newcommand{\eP}{\mathbf{P}}
\newcommand{\ber}{\mathsf{Ber}}

%%%%%%%%%% MDFRAMED ENVIORNMENT %%%%%%%
\definecolor{light-gray}{gray}{.90}
\newcommand{\red}[1]{{\color{red} #1}}

% \definecolor{light-red}{red}{.80}


%\newcommand{\methodname}{\textsf{MPR-Aware}}

\newmdenv[%
  backgroundcolor=SkyBlue!30, %
  linecolor=black,
  linewidth =1pt,%
  skipabove = 10pt,%
  skipbelow = 10pt
]{comment}

\newmdenv[%
  backgroundcolor=red, %
  linecolor=black,
  linewidth =1pt,%
  skipabove = 10pt,%
  skipbelow = 10pt
]{TODO}

\newcommand{\addref}{\red{[ADD REF]}}




%%%%%%%%%% Fancy Quotation %%%%%%%%%%%%%%
%%%%********************************************************************
\usepackage{microtype}
%%%%********************************************************************
% fancy quotes
\definecolor{quotemark}{gray}{0.7}
\makeatletter
\def\fquote{%
    \@ifnextchar[{\fquote@i}{\fquote@i[]}%]
           }%
\def\fquote@i[#1]{%
    \def\tempa{#1}%
    \@ifnextchar[{\fquote@ii}{\fquote@ii[]}%]
                 }%
\def\fquote@ii[#1]{%
    \def\tempb{#1}%
    \@ifnextchar[{\fquote@iii}{\fquote@iii[]}%]
                      }%
\def\fquote@iii[#1]{%
    \def\tempc{#1}%
    \vspace{1em}%
    \noindent%
    \begin{list}{}{%
         \setlength{\leftmargin}{0.1\textwidth}%
         \setlength{\rightmargin}{0.1\textwidth}%
                  }%
         \item[]%
         \begin{picture}(0,0)%
         \put(-15,-5){\makebox(0,0){\scalebox{3}{\textcolor{quotemark}{``}}}}%
         \end{picture}%
         \begingroup\itshape}%
 %%%%********************************************************************
 \def\endfquote{%
 \endgroup\par%
 \makebox[0pt][l]{%
 \hspace{0.8\textwidth}%
 \begin{picture}(0,0)(0,0)%
 \put(15,15){\makebox(0,0){%
 \scalebox{3}{\color{quotemark}''}}}%
 \end{picture}}%
 \ifx\tempa\empty%
 \else%
    \ifx\tempc\empty%
       \hfill\rule{100pt}{0.5pt}\\\mbox{}\hfill\tempa,\ \emph{\tempb}%
   \else%
       \hfill\rule{100pt}{0.5pt}\\\mbox{}\hfill\tempa,\ \emph{\tempb},\ \tempc%
   \fi\fi\par%
   \vspace{0.5em}%
 \end{list}%
 }%
 \makeatother
 %%%%********************************************************************

\newcommand{\dt}[1] {{\color{blue}[DT: #1]}}
\newcommand{\cl}[1] {{\color{violet}[CL: #1]}}
\newcommand{\hh}[1] {{\color{orange}[HH: #1]}}
\newcommand{\RC}[1] {{\color{red}[RC: #1]}}
% \newcommand{\fc}[1] {{\color{red}[FC: #1]}}
\newcommand{\noteC}[1]{ {\color{green} \textbf{CV:} #1} }


%%%%%%%%% Some of Dor's Macros:

\newcommand{\rB}{\mathrm{B}}
\newcommand{\rC}{\mathrm{C}}
\newcommand{\rE}{\mathrm{E}}
\newcommand{\rF}{\mathrm{F}}
\newcommand{\rG}{\mathrm{G}}
\newcommand{\rH}{\mathrm{H}}
\newcommand{\rh}{\mathrm{h}}
\newcommand{\rI}{\mathrm{I}}
\newcommand{\rJ}{\mathrm{J}}
\newcommand{\rK}{\mathrm{K}}
\newcommand{\rL}{\mathrm{L}}
\newcommand{\rM}{\mathrm{M}}
\newcommand{\rN}{\mathrm{N}}
\newcommand{\rO}{\mathrm{O}}
\newcommand{\rP}{\mathrm{P}}
\newcommand{\rQ}{\mathrm{Q}}
\newcommand{\rR}{\mathrm{R}}
\newcommand{\rS}{\mathrm{S}}
\newcommand{\rT}{\mathrm{T}}
\newcommand{\rU}{\mathrm{U}}
\newcommand{\rV}{\mathrm{V}}
\newcommand{\rW}{\mathrm{W}}
\newcommand{\rX}{\mathrm{X}}
\newcommand{\rY}{\mathrm{Y}}
\newcommand{\rZ}{\mathrm{Z}}
\newcommand{\sA}{\mathsf{A}}
\newcommand{\sB}{\mathsf{B}}
\newcommand{\sC}{\mathsf{C}}
\newcommand{\sE}{\mathsf{E}}
\newcommand{\sF}{\mathsf{F}}
\newcommand{\sG}{\mathsf{G}}
\newcommand{\sH}{\mathsf{H}}
\newcommand{\sh}{\mathsf{h}}
\newcommand{\sI}{\mathsf{I}}
\newcommand{\sJ}{\mathsf{J}}
\newcommand{\sK}{\mathsf{K}}
\newcommand{\sL}{\mathsf{L}}
\newcommand{\sM}{\mathsf{M}}
\newcommand{\sN}{\mathsf{N}}
\newcommand{\sO}{\mathsf{O}}
\newcommand{\sP}{\mathsf{P}}
\newcommand{\sQ}{\mathsf{Q}}
\newcommand{\sR}{\mathsf{R}}
\newcommand{\sS}{\mathsf{S}}
\newcommand{\sT}{\mathsf{T}}
\newcommand{\sD}{\mathsf{D}}
\newcommand{\sU}{\mathsf{U}}
\newcommand{\sV}{\mathsf{V}}
\newcommand{\sW}{\mathsf{W}}
\newcommand{\sX}{\mathsf{X}}
\newcommand{\sY}{\mathsf{Y}}
\newcommand{\sZ}{\mathsf{Z}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\FSG}{\mathcal{F}^{(\mathsf{SG})}_{d,K}}
\newcommand{\ui}{\underline{i}}
\newcommand{\skb}{s_{\mathsf{KB}}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\OO}{\mathbb{O}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\BS}{\mathbb{S}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}

==> preamble.tex <==
%!TEX root = main.tex

\usepackage[usenames,dvipsnames]{xcolor}
%\usepackage{mdframed}
%\usepackage{bm}
%\usepackage{bbm}
\usepackage{dsfont}
\usepackage{amsbsy}
\usepackage{amssymb}
\usepackage{amsmath}%
\usepackage{amsfonts}%
\usepackage{amsthm}
\usepackage{breqn}
\usepackage{graphicx}
\usepackage{colonequals}
\usepackage{psfrag}
\usepackage{mathrsfs}
\usepackage[noadjust]{cite}
\usepackage{hyperref}
\usepackage{mdframed}
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{braket}
\usepackage{mathtools}

\usepackage[backgroundcolor=blue!15]{todonotes}


%Enumitem setting
\newcommand\litem[1]{\item{\bfseries #1:}}


\allowdisplaybreaks

\newtheorem{thm}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{prop}{Proposition}
\newtheorem{conj}{Conjecture}
\newtheorem{cor}{Corollary}
\newtheorem{assumptions}{Assumption}
\newtheorem{question}{Question}

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother
\newreptheorem{conj}{Conjecture}

%% For watermarking
\newcommand{\rd}{R_d}
\newcommand{\rp}{R_p}
\newcommand{\Qx}{Q_X} % LLM distribution
\newcommand{\tilqs}{\tilde{Q}_{X|S}} % watermark distribution
\newcommand{\tilqBm}{\tilde{Q}_{X|B^m}} % watermark distribution
\newcommand{\tilqbm}{\tilde{Q}_{X|B^m=b^m}} % watermark distribution
\newcommand{\tilq}{\tilde{Q}_{X}} % marginalized watermarked distribution
\newcommand{\tilqBmi}{\tilde{Q}_{X|B^m=b^m_i}}

\newcommand{\pbm}{p(b^m)} %no rnadomness
\newcommand{\pBm}{p(B^m)} %random variable
\newcommand{\tpbm}{\tilde{p}(b^m)} %no rnadomness
\newcommand{\tpBm}{\tilde{p}(B^m)} %random variable

\newcommand{\pmu}{p_{\mu}} %random variable
\newcommand{\tpmu}{\tilde{p}_{\mu}} %random variable

%% Definition Styles
\theoremstyle{definition}
\newtheorem{quest}{Question}
\newtheorem{defn}{Definition}
\newtheorem{scheme}{Scheme}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
%%
\newcommand{\SNR}{\mbox{SNR}}
\newcommand{\dB}{\mbox{dB}}
\newcommand{\emu}{\colonsim}
\newcommand{\etal}{\textit{et al.}~}
\newcommand{\Fq}{\mathbb{F}_{q}}
%\newcommand{\PR}[1]{\mbox{Pr}\left\{ #1 \right\}}
\newcommand{\PR}{\mbox{Pr}}
\newcommand{\Lh}{\hat{l}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\Xk}{\mathcal{X}^k}
\newcommand{\Xn}{\mathcal{X}^n}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\mean}{\mathbb{E}}
\newcommand{\bc}{\mathbf{c}}

\newcommand{\fib}{f_{\mathsf{IB}}}
\newcommand{\fpf}{f_{\mathsf{PF}}}
\newcommand{\conv}{\mathsf{conv}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\rank}{\mbox{rank}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bbz}{\mathbf{z}}
\newcommand{\binstr}{\{0,1\}} 
\newcommand{\supp}{\mbox{supp}}
\renewcommand{\tilde}{\widetilde}
\newcommand{\Enc}{\mathsf{Enc}}
\newcommand{\Dec}{\mathsf{Dec}}
\newcommand{\Adv}{\mathsf{Adv}}
\newcommand{\chis}{\chi^2}
\newcommand{\Xh}{\hat{X}}
\newcommand{\Zh}{\hat{Z}}
\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\newcommand{\brk}[1]{\langle #1 \rangle}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\normQ}[1]{\| #1 \|_Q}
\newcommand{\normF}[1]{\| #1 \|_F}
\newcommand{\normX}[2]{\| #1 \|_{#2}}
\newcommand{\normEuc}[1]{\| #1 \|_2}
\newcommand{\ox}{\bar{x}}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\inertia}{\mathcal{I}}
\newcommand{\defined}{\triangleq}
\newcommand{\Tr}[1]{\mathrm{ tr}\left(#1 \right)}
\newcommand{\diag}[1]{\mathrm{diag}\left( #1 \right)}
\newcommand{\pxy}{P_{X,Y}}
\newcommand{\px}{P_X}
\newcommand{\py}{P_Y}
\newcommand{\pxp}{p_{X'}}
\newcommand{\pxgy}{P_{X|Y}}
\newcommand{\pygx}{P_{Y|X}}
\newcommand{\pbgx}{p_{B|X}}
\newcommand{\Ppygx}[1]{\mathbf{p}_{Y|X={#1}}}
\newcommand{\pxhgx}{p_{\Xh|X}}
\newcommand{\qx}{q_X}


\newcommand{\rx}{r_X}
\newcommand{\ExpVal}[2]{\mathbb{E}_{#1}\left[ #2 \right]}
\newcommand{\Mopt}{M_{\mathrm{ML}}}
\newcommand{\tZ}{\tilde{Z}}
\newcommand{\tU}{\tilde{U}}
\newcommand{\tV}{\tilde{V}}
\newcommand{\tsigma}{\tilde{\sigma}}
\newcommand{\Pxy}{\mathbf{P}_{X,Y}}
\newcommand{\Pxnyn}{P_{X^n,Y^n}}
\newcommand{\Pxyp}{P_{X',Y'}}
\newcommand{\Pygx}{\mathbf{P}_{Y|X}}
\newcommand{\Pxxp}{\bP_{X,\Xh}}
\newcommand{\Pxhgx}{P_{\hat{X}|X}}
\newcommand{\Px}{\mathbf{p}_X}
\newcommand{\Rx}{\mathbf{r}_X}
\newcommand{\Pxp}{\mathbf{p}_{\Xh}}
\newcommand{\Py}{\mathbf{p}_Y}
\newcommand{\At}{\tilde{\mathbf{A}}}
\newcommand{\Bt}{\tilde{\mathbf{B}}}
\newcommand{\Ut}{\tilde{\mathbf{U}}}
\newcommand{\Vt}{\mathbf{\tilde{V}}}
\newcommand{\Yt}{\tilde{Y}}
\newcommand{\Zt}{\tilde{Z}}
\newcommand{\lambdat}{\tilde{\lambda}}
\newcommand{\Sigmat}{\tilde{\mathbf{\Sigma}}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\Lb}{L}
\newcommand{\blambda}{\pmb{\lambda}}
\newcommand{\blambdat}{\tilde{\pmb{\lambda}}}
\newcommand{\bLambda}{\pmb{\Lambda}}
\newcommand{\Emat}{\mathbf{F}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\btu}{\tilde{\mathbf{u}}}
\newcommand{\btv}{\tilde{\mathbf{v}}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\tv}{\tilde{v}}
\newcommand{\olU}{\overline{\mathbf{U}}}
\newcommand{\deriv}[2]{\frac{\delta #1}{\delta #2}}
\newcommand{\sto}{\mbox{\normalfont s.t.}}
\newcommand{\KFnorm}[2]{\| #1 \|_{#2}}
\newcommand{\Imeas}{J}
\newcommand{\bigO}{O}
\newcommand{\ttheta}{\tilde{\theta}}
\newcommand{\Var}[2]{\mathrm{Var}_{#1}#2 }
\newcommand{\whf}{\widehat{f}}
\newcommand{\whg}{\widehat{g}}
\newcommand{\ft}{\tilde{f}}
\newcommand{\Yh}{\widehat{Y}}
%\newcommand{\pbgx}{p_{B|X^n}}
\newcommand{\pbgy}{p_{B|Y^n}}
\newcommand{\whh}{\widehat{h}}
% \newcommand{\EE}[1]{\ExpVal{}{#1}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\EM}[2]{\ExpVal{#1}{#2}}
\newcommand{\whB}{\widehat{B}}
\newcommand{\wbeta}{\widehat{\beta}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\eye}{\mathbf{I}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bSigma}{\mathbf{\Sigma}}
\newcommand{\bsigma}{\boldsymbol\sigma}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bbH}{\mathbf{H}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\suchthat}{\,\mid\,}
\newcommand{\indicator}{\mathds{1}}
\newcommand{\mmse}{\mathsf{mmse}}
\newcommand{\error}{\mathsf{e}}
%%
\newcommand{\calN}{\mathcal{N}}
\newcommand{\cwd}{\{1,\dots,2^{nR} \}}
\newcommand{\Ps}{\mathbf{p}_S}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\TV}{\mathsf{TV}}
\newcommand{\lse}{\mathsf{lmmse}}
\newcommand{\dks}{d_{\mathrm{KS}}}
\newcommand{\Xt}{\widetilde{X}}
\newcommand{\xh}{\hat{x}}
\newcommand{\vs}{v^*(p_{S,X})}
\newcommand{\dps}{\delta(p_{S,X})}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\simplex}{\Delta}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\KC}{\calJ}
\newcommand{\Fsym}{\calF_{\mathrm{sym}}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\Dx}{\mathbf{D}_X}
\newcommand{\Dy}{\mathbf{D}_Y}
\newcommand{\Dkl}{\mathsf{D}_{\mathsf{KL}}}
\newcommand{\pdset}{\calP^m_{++}}
\newcommand{\eP}{\mathbf{P}}
\newcommand{\ber}{\mathsf{Ber}}

%%%%%%%%%% MDFRAMED ENVIORNMENT %%%%%%%
\definecolor{light-gray}{gray}{.90}
\newcommand{\red}[1]{{\color{red} #1}}

% \definecolor{light-red}{red}{.80}


%\newcommand{\methodname}{\textsf{MPR-Aware}}

\newmdenv[%
  backgroundcolor=SkyBlue!30, %
  linecolor=black,
  linewidth =1pt,%
  skipabove = 10pt,%
  skipbelow = 10pt
]{comment}

\newmdenv[%
  backgroundcolor=red, %
  linecolor=black,
  linewidth =1pt,%
  skipabove = 10pt,%
  skipbelow = 10pt
]{TODO}

\newcommand{\addref}{\red{[ADD REF]}}




%%%%%%%%%% Fancy Quotation %%%%%%%%%%%%%%
%%%%********************************************************************
\usepackage{microtype}
%%%%********************************************************************
% fancy quotes
\definecolor{quotemark}{gray}{0.7}
\makeatletter
\def\fquote{%
    \@ifnextchar[{\fquote@i}{\fquote@i[]}%]
           }%
\def\fquote@i[#1]{%
    \def\tempa{#1}%
    \@ifnextchar[{\fquote@ii}{\fquote@ii[]}%]
                 }%
\def\fquote@ii[#1]{%
    \def\tempb{#1}%
    \@ifnextchar[{\fquote@iii}{\fquote@iii[]}%]
                      }%
\def\fquote@iii[#1]{%
    \def\tempc{#1}%
    \vspace{1em}%
    \noindent%
    \begin{list}{}{%
         \setlength{\leftmargin}{0.1\textwidth}%
         \setlength{\rightmargin}{0.1\textwidth}%
                  }%
         \item[]%
         \begin{picture}(0,0)%
         \put(-15,-5){\makebox(0,0){\scalebox{3}{\textcolor{quotemark}{``}}}}%
         \end{picture}%
         \begingroup\itshape}%
 %%%%********************************************************************
 \def\endfquote{%
 \endgroup\par%
 \makebox[0pt][l]{%
 \hspace{0.8\textwidth}%
 \begin{picture}(0,0)(0,0)%
 \put(15,15){\makebox(0,0){%
 \scalebox{3}{\color{quotemark}''}}}%
 \end{picture}}%
 \ifx\tempa\empty%
 \else%
    \ifx\tempc\empty%
       \hfill\rule{100pt}{0.5pt}\\\mbox{}\hfill\tempa,\ \emph{\tempb}%
   \else%
       \hfill\rule{100pt}{0.5pt}\\\mbox{}\hfill\tempa,\ \emph{\tempb},\ \tempc%
   \fi\fi\par%
   \vspace{0.5em}%
 \end{list}%
 }%
 \makeatother
 %%%%********************************************************************

\newcommand{\dt}[1] {{\color{blue}[DT: #1]}}
\newcommand{\cl}[1] {{\color{violet}[CL: #1]}}
\newcommand{\hh}[1] {{\color{orange}[HH: #1]}}
% \newcommand{\fc}[1] {{\color{red}[FC: #1]}}
\newcommand{\noteC}[1]{ {\color{green} \textbf{CV:} #1} }


%%%%%%%%% Some of Dor's Macros:

\newcommand{\rB}{\mathrm{B}}
\newcommand{\rC}{\mathrm{C}}
\newcommand{\rE}{\mathrm{E}}
\newcommand{\rF}{\mathrm{F}}
\newcommand{\rG}{\mathrm{G}}
\newcommand{\rH}{\mathrm{H}}
\newcommand{\rh}{\mathrm{h}}
\newcommand{\rI}{\mathrm{I}}
\newcommand{\rJ}{\mathrm{J}}
\newcommand{\rK}{\mathrm{K}}
\newcommand{\rL}{\mathrm{L}}
\newcommand{\rM}{\mathrm{M}}
\newcommand{\rN}{\mathrm{N}}
\newcommand{\rO}{\mathrm{O}}
\newcommand{\rP}{\mathrm{P}}
\newcommand{\rQ}{\mathrm{Q}}
\newcommand{\rR}{\mathrm{R}}
\newcommand{\rS}{\mathrm{S}}
\newcommand{\rT}{\mathrm{T}}
\newcommand{\rU}{\mathrm{U}}
\newcommand{\rV}{\mathrm{V}}
\newcommand{\rW}{\mathrm{W}}
\newcommand{\rX}{\mathrm{X}}
\newcommand{\rY}{\mathrm{Y}}
\newcommand{\rZ}{\mathrm{Z}}
\newcommand{\sA}{\mathsf{A}}
\newcommand{\sB}{\mathsf{B}}
\newcommand{\sC}{\mathsf{C}}
\newcommand{\sE}{\mathsf{E}}
\newcommand{\sF}{\mathsf{F}}
\newcommand{\sG}{\mathsf{G}}
\newcommand{\sH}{\mathsf{H}}
\newcommand{\sh}{\mathsf{h}}
\newcommand{\sI}{\mathsf{I}}
\newcommand{\sJ}{\mathsf{J}}
\newcommand{\sK}{\mathsf{K}}
\newcommand{\sL}{\mathsf{L}}
\newcommand{\sM}{\mathsf{M}}
\newcommand{\sN}{\mathsf{N}}
\newcommand{\sO}{\mathsf{O}}
\newcommand{\sP}{\mathsf{P}}
\newcommand{\sQ}{\mathsf{Q}}
\newcommand{\sR}{\mathsf{R}}
\newcommand{\sS}{\mathsf{S}}
\newcommand{\sT}{\mathsf{T}}
\newcommand{\sD}{\mathsf{D}}
\newcommand{\sU}{\mathsf{U}}
\newcommand{\sV}{\mathsf{V}}
\newcommand{\sW}{\mathsf{W}}
\newcommand{\sX}{\mathsf{X}}
\newcommand{\sY}{\mathsf{Y}}
\newcommand{\sZ}{\mathsf{Z}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\FSG}{\mathcal{F}^{(\mathsf{SG})}_{d,K}}
\newcommand{\ui}{\underline{i}}
\newcommand{\skb}{s_{\mathsf{KB}}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\OO}{\mathbb{O}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\BS}{\mathbb{S}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}
